Neural Skill Transfer from Supervised Language Tasks to Reading Comprehension

Reading comprehension is a challenging task in natural language processing and requires a set of skills to be solved. While current approaches focus on solving the task as a whole, in this paper, we propose to use a neural network `skill' transfer approach. We transfer knowledge from several lower-level language tasks (skills) including textual entailment, named entity recognition, paraphrase detection and question type classification into the reading comprehension model. We conduct an empirical evaluation and show that transferring language skill knowledge leads to significant improvements for the task with much fewer steps compared to the baseline model. We also show that the skill transfer approach is effective even with small amounts of training data. Another finding of this work is that using token-wise deep label supervision for text classification improves the performance of transfer learning.

==> abstract.tex <==
Reading comprehension is a challenging task in natural language processing and requires a set of skills to be solved. While current approaches focus on solving the task as a whole, in this paper, we propose to use a neural network `skill' transfer approach. We transfer knowledge from several lower-level language tasks (skills) including textual entailment, named entity recognition, paraphrase detection and question type classification into the reading comprehension model.
 We conduct an empirical evaluation and show that transferring language skill knowledge leads to significant improvements for the task with much fewer steps compared to the baseline model. We also show that the skill transfer approach is effective even with small amounts of training data.
Another finding of this work is that using token-wise deep label supervision for text classification improves the performance 
of transfer learning.

==> sec_data.tex <==
\section{Data and Tasks}
\label{sec:data-and-tasks}
SQUAD\\
Textual Entailment\\
PPDB\\
Question Type Classification\\



==> sec_s_acknowledge.tex <==
\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments go at the end of the paper. Do not include
acknowledgments in the anonymized submission, only in the final paper.

==> tables/comb-skill-tasks-qa-skill.tex <==
\resizebox{\linewidth}{!}{
\minipage{0.45\linewidth}
\centering
\input{tables/qa-skill-ablations-squad}
% \caption{SRL results.}
% \label{tbl:results_srl}
\endminipage\hfill
\minipage{0.45\linewidth}
\centering
\input{tables/skill-tasks-train-results}
\endminipage\hfill
}

==> tables/skill-tasks-train-results.tex <==
\begin{table*}[]
\centering
\begin{tabular}{@{}lccc@{}}
\textbf{Task}  & \textbf{Dataset} & \textbf{Test} & \textbf{SOA} \\ \hline
TE & SNLI 1.0 & 83.61 & 88.0 \cite{Gong2017-te-interaction-cnn} \\
 Paraphrase & PPDB 2.0, S & 75.3 & - \\ \hline
NER& Conll 2012& 74.3 & \\ \hline
QTC$_{sent label}$& TREC-QC  & 83.2 & \multirow{2}{*}{88.0}\\
QTC$_{token label}$& TREC-QC  & 85.8 &\\ \hline
\end{tabular}
\caption{Experiments with different Skill models on their evaluation datasets.} 
\label{table:skill-tasks}
\end{table*}

% \begin{table*}[]
% \centering
% \begin{tabular}{@{}lccc@{}}
%  \textbf{Task type} & \textbf{Task}  & \textbf{Dataset} & \textbf{Test} \\ \hline
% \multirow{2}{*}{Relation Classification}                  & Textual Entailment                       & SNLI 1.0                    & 83.61                    \\
%                                      & Paraphrase                               & PPDB 2.0, small             & 75.3                     \\ \hline
% Sequence Labeling                               & Named Entity Recognition                 & Conll 2012                  & 74.3                     \\ \hline
% \multirow{2}{*}{Text classification} & \multirow{2}{*}{Question \textcolor{blue}{Type} Classification} & TREC-QC – sent label supervision    & 83.2                     \\
%                                      &                                          & TREC-QC – token deep supervision    & 85.8                     \\ \hline
% \end{tabular}
% \caption{Experiments with different Skill models on their evaluation datasets. `-' means that no dev set is available.
% %the dataset does not provide a dev set.
% In such a case we train for a fixed number of epochs and
% % present
% \textcolor{blue}{use the resulting score.}}
% \label{table:skill-tasks}
% \end{table*}
